Multi-label Chaining with Imprecise Probabilities

We present two different strategies to extend the classical multi-label chaining approach to handle imprecise probability estimates. These estimates use convex sets of distributions (or credal sets) in order to describe our uncertainty rather than a precise one. The main reasons one could have for using such estimations are (1) to make cautious predictions (or no decision at all) when a high uncertainty is detected in the chaining and (2) to make better precise predictions by avoiding biases caused in early decisions in the chaining. We adapt both strategies to the case of the naive credal classifier, showing that this adaptations are computationally efficient. Our experimental results on missing labels, which investigate how reliable these predictions are in both approaches, indicate that our approaches produce relevant cautiousness on those hard-to-predict instances where the precise models fail.

==> multi-label chaining with imprecise probabilities/images/marginalization_general_from.tex <==
\tikzset{
  treenode/.style = {shape=rectangle, rounded corners,
                     draw, align=center,
                     top color=white, 
                     bottom color=blue!20},
  root/.style     = {treenode, 
  		font=\Large, bottom color=black!30},
  one/.style      = {treenode, 
  		  minimum size=4mm,
		 inner sep=0pt, outer sep=0pt,
  		 shape=circle,
  		 bottom color=red!30,
  		 top color=white,
  		 align=center,
  		 font=\ttfamily\normalsize},
  zero/.style      = {treenode, 
  		 minimum size=4mm,
		 inner sep=0pt, outer sep=0pt,
		 shape=circle,
		 top color=white,
  		 align=center,
  		 font=\ttfamily\normalsize},	
  imprecise/.style      = {treenode, 
  		 minimum size=4mm,
		 inner sep=0pt, outer sep=0pt,
		 shape=circle,
		 bottom color=green!30,
		 top color=white,
  		 align=center,
  		 font=\ttfamily\normalsize},		 
  cross/.style={cross out, draw=black, solid, 
  	thick, minimum size=1.5*(#1-\pgflinewidth), 
  	inner sep=1.5, outer sep=0pt},
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Set the overall layout of the tree
\tikzstyle{level 1}=[level distance=0.8cm, sibling distance=0.8cm]
\tikzstyle{level 2}=[level distance=0.8cm, sibling distance=0.8cm]
\tikzstyle{level 3}=[level distance=0.8cm, sibling distance=0.8cm]
\tikzstyle{level 4}=[level distance=0.8cm, sibling distance=0.8cm]
\tikzstyle{level 5}=[level distance=0.8cm, sibling distance=0.8cm]
% Define styles for bags and leafs
\tikzstyle{bag} = [text width=4em, text centered]
\tikzstyle{end} = [circle, minimum width=3pt,fill, inner sep=0pt]
\tikzstyle{pruned} = [cross, minimum width=3pt,fill, inner sep=0pt]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tikzpicture}[
	grow=right, 
	sloped,
	edge from parent/.style = 
		{draw, font=\tiny\sffamily, text=blue},
	every node/.style = {font=\footnotesize}	]
\node(r)[root] {}
    child {
        node (1)[cross] {}        
        edge from parent 
        node[below] {}
    }
    child {
        node(2)[imprecise]{*}
        child {
            node(21)[one] {1}
            child {
            	node(211)[cross] {}
            }
            child {
        		node(212)[imprecise]{*}
        		child {
	              node(2121)[one,
	              		label=right:{\tred{\bf $(*, 1, *, ?)$}}] {1}    
	            }
	            child {
     			   node(2122)[cross]{}
			    }
	            child {
	              node(2120)[cross] {}
	            }
    		}
            child {
           		node(210)[cross]{}
            	edge from parent
            	node[above] {}
           }
        }
        child {
            node(02)[cross]{}
        }
        child {
            node(00)[cross]{}
            edge from parent
            node[above] {}
        }
        edge from parent         
        node[above] {}
    }
    child {
        node(0)[cross]{}
    };
\draw[dashed,->, bend left, red]  (r) to (2);
\draw[dashed,->, bend left, red] (2) to (21);
\draw[dashed,->, bend right, red] (21) to (212);
\draw[dashed,->, bend right, red] (212) to (2121);

\node[yshift=12pt, xshift=1pt] at (2) {$Y_1$};
\node[yshift=-12pt, xshift=1pt] at (21) {$Y_2$};
\node[yshift=12pt, xshift=1pt] at (212) {$Y_3$};
\node[yshift=-12pt, xshift=1pt] at (2121) {$Y_4$};
\end{tikzpicture}







==> multi-label chaining with imprecise probabilities/images/marginalization_general_from_ncc.tex <==
\tikzset{
  treenode/.style = {shape=rectangle, rounded corners,
                     draw, align=center,
                     top color=white, 
                     bottom color=blue!20},
  root/.style     = {treenode, 
  		font=\Large, bottom color=black!30},
  one/.style      = {treenode, 
  		  minimum size=4mm,
		 inner sep=0pt, outer sep=0pt,
  		 shape=circle,
  		 bottom color=red!30,
  		 top color=white,
  		 align=center,
  		 font=\ttfamily\normalsize},
  zero/.style      = {treenode, 
  		 minimum size=4mm,
		 inner sep=0pt, outer sep=0pt,
		 shape=circle,
		 top color=white,
  		 align=center,
  		 font=\ttfamily\normalsize},	
  imprecise/.style      = {treenode, 
  		 minimum size=4mm,
		 inner sep=0pt, outer sep=0pt,
		 shape=circle,
		 bottom color=green!30,
		 top color=white,
  		 align=center,
  		 font=\ttfamily\normalsize},		 
  cross/.style={cross out, draw=black, solid, 
  	thick, minimum size=1.5*(#1-\pgflinewidth), 
  	inner sep=1.5, outer sep=0pt},
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Set the overall layout of the tree
\tikzstyle{level 1}=[level distance=0.8cm, sibling distance=1.2cm]
\tikzstyle{level 2}=[level distance=0.8cm, sibling distance=0.8cm]
\tikzstyle{level 3}=[level distance=0.8cm, sibling distance=0.8cm]
\tikzstyle{level 4}=[level distance=0.8cm, sibling distance=0.8cm]
\tikzstyle{level 5}=[level distance=0.8cm, sibling distance=0.8cm]
% Define styles for bags and leafs
\tikzstyle{bag} = [text width=4em, text centered]
\tikzstyle{end} = [circle, minimum width=3pt,fill, inner sep=0pt]
\tikzstyle{pruned} = [cross, minimum width=3pt,fill, inner sep=0pt]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tikzpicture}[
	grow=right, 
	sloped,
	edge from parent/.style = 
		{draw, font=\tiny\sffamily, text=blue},
	every node/.style = {font=\footnotesize}	]
\node(r)[root] {}
    child {
        node(1)[one] {1}        
        child {
           node(11)[one, label=right:{\tred{\bf $(*, 1, *, ?)$}}] {1}
        }
        child {
        	node(12)[cross]{}
    	}
        child {
           node(10)[cross]{}
           edge from parent
           node[above] {}
        }
    }
    child {
        node(0)[cross] {}  
    };
\draw[dashed,->, bend left, red]  (r) to (1);
\draw[dashed,->, bend left, red] (1) to (11);
\node[yshift=12pt, xshift=1pt] at (1) {$Y_2$};
\node[yshift=-12pt, xshift=1pt] at (11) {$Y_4$};

\end{tikzpicture}







==> multi-label chaining with imprecise probabilities/suplementary_proofs.tex <==
\newpage
\appendix
\section*{Appendix}
%{\Large Supplementary materials are given for reviewer convenience and the sake of exhaustivity. They will be removed in the final version to respect space limits.}
\section{NCC derivation for multi-label chaining}
As the purpose of the imprecise chaining is to compute binary conditional dependence models, we need only get conditional probability bounds of the probability $P(Y_{j}=y_j|\mathbf{X}=\newinstance, Y_{\setindices^{j-1}}\!\!=\hat{\vect{y}}_{\setindices^{j-1}})$, so by using Bayes' theorem and naive Bayes' attribute independence assumption, it can be written as follows
\begin{align}\label{eq:marginalbayeschain}\!\!
\frac{P(Y_{j}=y_j)
	\prod_{i=1}^p  P(X_i = x_i|Y_{j}=y_j)
	\prod_{k=1}^{j-1} 
		P(Y_{k}\!\!=\hat{y}_{k}|Y_{j}=y_j)
}{\sum_{y_l\in\{0, 1\}}P(Y_{j}=y_l)
	\prod_{i=1}^p  P(X_i = x_i|Y_{j}=y_l)
	\prod_{k=1}^{j-1} 
		P(Y_{k}\!\!=\hat{y}_{k}|Y_{j}=y_l)
}.
\end{align}

Computing lower and upper probability bounds $[\underline{P},\overline{P}]$ over all possible marginals $\credal_{Y_j}$ and conditional distributions $\credal_{X_i|Y_j}, \credal_{Y_k|Y_j}$ can be performed by solving the following minimization/maximization problem of Equation~\eqref{eq:marginalbayeschain} as follows
\begin{align}
\underline{P}(Y_{j}=y_j|&X\!\!=\!\newinstance, Y_{\setindices^{j-1}}\!\!=\!\hat{\bm{y}}_{\setindices^{j-1}}) =\nonumber\\
&\min_{P\in\credal_{Y_j}} \min_{\substack{P\in\left\{\credal_{X_i|Y_j},\credal_{Y_k|Y_j}\right\}\\i=1,\dots,d\\k=1,\dots, j-1}} P(Y_{j}=y_j|X\!\!=\!\newinstance,Y_{\setindices^{j-1}}\!\!=\!\hat{\bm{y}}_{\setindices^{j-1}}),\\
\overline{P}(Y_{j}=y_j|&X\!\!=\!\newinstance,Y_{\setindices^{j-1}}\!\!=\!\hat{\bm{y}}_{\setindices^{j-1}}) =\nonumber\\
&\max_{P\in\credal_{Y_j}} \max_{\substack{P\in\left\{\credal_{X_i|Y_j},\credal_{Y_k|Y_j}\right\}\\i=1,\dots,d\\k=1,\dots, j-1}} P(Y_{j}=y_j|X\!\!=\!\newinstance,Y_{\setindices^{j-1}}\!\!=\!\hat{\bm{y}}_{\setindices^{j-1}}).
\end{align}

In practice, we assume a precise estimation of the marginal distribution $\mathbb{P}_{Y_j}$ in lieu of a credal set $\credal_{Y_j}$, so  optimization problems over the credal set of marginal distributions $\credal_{Y_j}$ can be ignored. Therefore, one can easily show that last equations evaluated to $Y_{j}=1$ ($Y_{j}=0$ can be directly calculated using duality) are equivalent to 
\begin{align}
	\underline{P}(Y_{j}\eq1|
		\mathbf{X}\eq\newinstance, 
		Y_{\setindices^{j-1}}=\hat{\bm{y}}_{\setindices^{j-1}}) &\eq
		\left(\!1+ \frac{P(Y_{j}\eq0)
				\overline{P}_{0}(\mathbf{X}\eq{\newinstance})
				\overline{P}_{0}(Y_{\setindices^{j-1}}\eq
					\hat{\bm{y}}_{\setindices^{j-1}})
			}
			{P(Y_{j}\eq1)
				\underline{P}_{1}(\mathbf{X}\eq{\newinstance})
				\underline{P}_{1}(Y_{\setindices^{j-1}}\eq
					\hat{\bm{y}}_{\setindices^{j-1}})
			}
		\!\right)^{-1}\!\!\! \label{eq:ncclowerproof} \\
	\!\!\!\overline{P}(Y_{j}\eq1| \mathbf{X}
		\eq\newinstance, Y_{\setindices^{j-1}}\eq
			\hat{\bm{y}}_{\setindices^{j-1}}) &\eq
		\left(\!1+ \frac{P(Y_{j}=0)
			\underline{P}_{0}(\mathbf{X}\eq{\newinstance})
				\underline{P}_{0}(Y_{\setindices^{j-1}}\eq
					\hat{\bm{y}}_{\setindices^{j-1}})
			}
			{P(Y_{j}\eq1)
				\overline{P}_{1}(\mathbf{X}={\newinstance})
					\overline{P}_{1}(Y_{\setindices^{j-1}}\eq
						\hat{\bm{y}}_{\setindices^{j-1}})
			}
		\!\right)^{-1}\!\!\!\!\! \label{eq:nccupperproof}
\end{align}
where probability bounds $[\underline{P}_{1}, \overline{P}_{1}]$ and $[\underline{P}_{0}, \overline{P}_{0}]$ of each different conditional event are defined as follows
{\small\begin{align}
	\overline{P}_{0}(\mathbf{X}=\newinstance)\!:=\!
		\prod_{i=1}^p \overline{P}(X_i = x_i|Y_{j}\eq0)
	~~&\text{and}~~
	\overline{P}_{0}(\mathbf{Y}_{\setindices^{j-1}}=
			\vect{y}_{\setindices^{j-1}})\!:=\!
		\prod_{k=1}^{j-1} \overline{P}(Y_k=\hat{y}_k|Y_{j}\eq0),
	\label{eq:ncclabelupperproof}
	\\
	\underline{P}_{1}(\mathbf{X}=\newinstance)\!:=\!
		\prod_{i=1}^p \underline{P}(X_i = x_i|Y_{j}\eq1)
	~~&\text{and}~~
	\underline{P}_{1}(\mathbf{Y}_{\setindices^{j-1}}=
			\vect{y}_{\setindices^{j-1}})\!:=\!
		\prod_{k=1}^{j-1} \underline{P}(Y_k=\hat{y}_k|Y_{j}\eq1).
	\label{eq:ncclabellowerproof}
\end{align}}

The last conditional probability bounds are derived using the Imprecise Dirichlet model (IDM)~\cite{walley1996inferences}
\begin{align}\label{eq:nccidm}
	\underline{P}(X_i\eq x_i| Y_{j}\eq y_j)\eq  
		\frac{n(x_i|y_j)}{n(y_j)+s}
	~~\text{and}~~
	\overline{P}(X_i\eq x_i| Y_{j}\eq y_j)\eq 
		\frac{n(x_i|y_j)+s}{n(y_j)+s}
\end{align}
where $n(\cdot)$ is a count function that counts the number of occurrences of events $x_i|y_j$ and $y_j$ in the observed data set. For instance; $n(x_i|y_j)$ is the number of instances in the training set where $X_i=x_i$ and the label value is $Y_i=y_i$. 

In the same way as precedent equations, we can obtain probability bounds $[\underline{P}(Y_k=\hat{y}_k|Y_{j}=y_j), \overline{P}(Y_k=\hat{y}_k|Y_{j}=y_j)]$.

\begin{remark}
	The denominator of Equations \eqref{eq:ncclowerproof} and \eqref{eq:nccupperproof} may in some cases (depending on the training data) become zero, and therefore, the division would not be defined. In these cases, we adopt the ``Laplace smoothing'' technique for the precise probabilities $P(Y_{j}=0)$ and $P(Y_{j}=1)$. Furthermore, if we obtain an undefined division, i.e. $0/0$, we manually put $0$.
\end{remark}

\begin{remark}
	Note that the choice of the marginal distribution $\mathbb{P}_{Y_j}$ in lieu of a credal set $\credal_{Y_j}$ does not change the theoretical results obtained in Proposition~\ref{prop:nccib}. However, if the credal $\mathscr{P}_Y$ is considered, we can obtain a very small, but not significant, improvement in the experimental results\footnote{Anyone can reproduce these results by using our online implementation.}.
\end{remark}


\section{Proofs for our results}
\begin{proof}[\textbf{of Proposition~\ref{prop:nccib}}]
Let us begin to prove the optimization problem of the lower probability of \eqref{eq:impbranching} evaluated to $Y_j=1$
\begin{equation}
\lowercondprobchain(Y_j=1) = 
\min_{\vect{y}\in\{0,1\}^{\left|\setindices_{\mathcal{A}}^{j-1}\right|}} 
	\underline{P}_{\newinstance}(Y_j=1|
		Y_{\setindices_\mathcal{R}^{j-1}}=1, 
		Y_{\setindices_{\mathcal{I}}^{j-1}}=0,
		Y_{\setindices_{\mathcal{A}}^{j-1}}=\vect{y}).
\end{equation}
Let us to define $\setindices^{j-1}_*=\setindices_{\mathcal{R}}^{j-1}\cup\setindices_{\mathcal{I}}^{j-1}$ as the set of indices of relevant and irrelevant predicted labels down to the $(j-1){th}$ index. By applying Equation~\eqref{eq:ncclowerproof} to the right side of last equation, we get 
\begin{equation*}
	\min_{\vect{y}\in\{0,1\}^{\left|\setindices_{\mathcal{A}}^{j-1}\right|}} 
	\left(1+ \frac{P(Y_{j}=0)
				\overline{P}_{0}(\mathbf{X}={\newinstance})
				\overline{P}_{0}(Y_{\setindices^{j-1}_*}=
					\hat{\bm{y}}_{\setindices^{j-1}_*},
				Y_{\setindices_\mathcal{A}^{j-1}}=\vect{y})
			}
			{P(Y_{j}=1)
				\underline{P}_{1}(\mathbf{X}={\newinstance})
				\underline{P}_{1}(Y_{\setindices^{j-1}_*}=
					\hat{\bm{y}}_{\setindices^{j-1}_*},
				Y_{\setindices_\mathcal{A}^{j-1}}=\vect{y})
			}
	\right)^{-1},
\end{equation*}
where $\hat{\bm{y}}_{\setindices^{j-1}_*}$ is the binary vector with predicted relevant and irrelevant values. So, using the fact that minimizing $\frac{1}{1+x}$ is equal to maximizing $x$, we therefore get 
\begin{equation*}
	\max_{\vect{y}\in\{0,1\}^{\left|\setindices_{\mathcal{A}}^{j-1}\right|}} 
	\frac{P(Y_{j}=0)
		\overline{P}_{0}(\mathbf{X}={\newinstance})
		\overline{P}_{0}(Y_{\setindices^{j-1}_*}=
			\hat{\bm{y}}_{\setindices^{j-1}_*})
		\overline{P}_{0}(Y_{\setindices_\mathcal{A}^{j-1}}=
			\vect{y})
	}
	{P(Y_{j}=1)
		\underline{P}_{1}(\mathbf{X}={\newinstance})
		\underline{P}_{1}(Y_{\setindices^{j-1}_*}=
			\hat{\bm{y}}_{\setindices^{j-1}_*})
		\underline{P}_{1}(Y_{\setindices_\mathcal{A}^{j-1}}=
			\vect{y})
	}.
\end{equation*}
%The first three terms of the numerator (and of the denominator) of the last equation can be considered as constants, and therefore these can be omitted from t. he optimization problem since they do not change the optimal solution.

The first three terms of the numerator (and of the denominator) of the last equation can be omitted from the optimization problem since they do not change the optimal solution, and by applying Equations~ \eqref{eq:ncclabelupperproof}, \eqref{eq:ncclabellowerproof} and \eqref{eq:nccidm}, to the last term, we get what we sought
\begin{align*}
	&\max_{\vect{y}\in\{0,1\}^{\left|\setindices_{\mathcal{A}}^{j-1}\right|}} 
	\frac{\overline{P}_{0}(Y_{\setindices_\mathcal{A}^{j-1}}=
			\vect{y})}
	{\underline{P}_{1}(Y_{\setindices_\mathcal{A}^{j-1}}=
			\vect{y})} \\
	%%%%%%%%%%%%%%%%%%%%
	\iff & \max_{\vect{y}\in\{0,1\}^{\left|\setindices_{\mathcal{A}}^{j-1}\right|}} 
	\frac{\prod_{k\in\setindices_\mathcal{A}^{j-1}} \overline{P}(Y_k=y_k|Y_{j}\eq0)}
	{\prod_{k\in\setindices_\mathcal{A}^{j-1}} \underline{P}(Y_k=y_k|Y_{j}\eq1)}\\
	%%%%%%%%%%%%%%%%%%%%
	\iff &\max_{\vect{y}\in\{0,1\}^{\left|\setindices_{\mathcal{A}}^{j-1}\right|}} 
		\frac{\prod_{k\in\setindices_\mathcal{A}^{j-1}}\frac{n(y_k|y_j=0)+s}{n(y_j=0)+s}}
		{\prod_{k\in\setindices_\mathcal{A}^{j-1}}\frac{n(y_k|y_j=1)}{n(y_j=1)+s}}\\
	%%%%%%%%%%%%%%%
	\iff &\max_{\vect{y}\in\{0,1\}^{\left|\setindices_{\mathcal{A}}^{j-1}\right|}} 
	\left[\frac{n(y_j=1)+s}{n(y_j=0)+s}
		\right]^{\left|\setindices_{\mathcal{A}}^{j-1}\right|}
	\prod_{y_i\in\vect{y}}^{~~i\in\setindices_{\mathcal{A}}^{j-1}}
		\frac{n(y_i|y_j=0)+s}{n(y_i|y_j=1)},
\end{align*}
in which it is easy see that: (1) the term $[\cdots]^{\left|\setindices_{\mathcal{A}}^{j-1}\right|}$ can be omitted, and hence, we can get $\hat{\underline{\vect{y}}}_{\setindices_{\mathcal{A}}^{j-1}}$, and (2) using similar arguments as above we can easily get the labels $\hat{\overline{\vect{y}}}_{\setindices_{\mathcal{A}}^{j-1}}$ which maximise the upper probability $\overline{P}_{\newinstance}(Y_j=1)$ of \eqref{eq:impbranching}.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mbox{}\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}[\textbf{of Proposition~\ref{prop:ibcomplexity}}]
	This proof can be performed using a dichotomy algorithm (equivalent to a binary search tree), starting with $y_{k}$ last abstained label (i.e. $k=|\setindices_{\mathcal{A}}|-1$) and calculating the values $\frac{n(y_k=1|\cdot)+s}{n(y_k=1|\cdot)}$ and $\frac{n(y_k=0|\cdot)+s}{n(y_k=0|\cdot)}$, then we retain the maximal value of these last two terms (or the minimal value, whichever applies) and we go forward with second-to-last label $y_{k-1}$, but this time multiplied by the last term retained, and so on. After having obtained the lower binary path $\hat{\underline{\vect{y}}}_{\setindices_{\mathcal{A}}^{j-1}}$(or the upper binary path $\hat{\overline{\vect{y}}}_{\setindices_{\mathcal{A}}^{j-1}}$), we can directly calculate the values $\lowercondprobchain(Y_j=1)$ and $\uppercondprobchain(Y_j=1)$ (and by duality of the lower and upper probability bounds $[\lowercondprobchain(Y_j=0), \uppercondprobchain(Y_j=0)]$).
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mbox{}\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}[\textbf{of Proposition~\ref{prop:globalcomplexity}}]
The proof for the best-case is straighforward, because if there is not any abstained labels, the time complexity is the same than precise chaining $\mathcal{O}(m)$. The worst-case complexity, in which all inferred labels are abstained, is also easy to calculate: the first label performs a single operation, i.e. $\mathcal{O}(1)$, then the second label is also inferred in a single operation due to the number of previous abstained labels being equal to $1$ (c.f. Proposition~\ref{prop:ibcomplexity}), then the third label takes into account two previous abstained labels and performs two operations (c.f. Proposition~\ref{prop:ibcomplexity}), and the fourth label performs three operations, and so on. We therefore obtain $\mathcal{O}(\nicefrac{m(m-1)}{2}+1)$ operations which is equal to $\mathcal{O}(m^2)$ asymptotically.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
\section{Supplementary results}

\begin{figure}[!th]
	\centering
	\subfigure[\sc Emotions]{\hspace{-2mm}
	   \includegraphics[width=0.33\linewidth]{images/missing/emotions_mar_disc6}
	}%
	\subfigure[\sc Enron]{\hspace{-1mm}
		\includegraphics[width=0.33\linewidth]{images/missing/enron_mar_disc6}
	}%
	\subfigure[\sc Yeast]{\hspace{-1mm}
		\includegraphics[width=0.33\linewidth]{images/missing/yeast_mar_disc6}
	}\quad%
	\subfigure[\sc Scene]{\hspace{-2mm}
	   \includegraphics[width=0.33\linewidth]{images/missing/scene_mar_disc6}
	}%
	\subfigure[\sc Medical]{\hspace{-1mm}
		\includegraphics[width=0.33\linewidth]{images/missing/medical_mar_disc6}
	}%
	\subfigure[\sc CAL500]{\hspace{-1mm}
		\includegraphics[width=0.33\linewidth]{images/missing/cal500_mar_disc6}
	}%
	\caption{\textbf{Missing labels - Marginalization} Evolution of the average (\%) set-accuracy (top) and completeness (down) for each level of imprecision (a curve for each one) and discretization $z=6$, with respect the percentage of missing labels.}
\end{figure}


\begin{figure}[!th]
	\vspace{-4mm}\centering
	\subfigure[\sc Scene]{\hspace{-2mm}
	   \includegraphics[width=0.33\linewidth]{images/missing/emotions_ib_disc6}
	}%
	\subfigure[\sc Medical]{\hspace{-1mm}
		\includegraphics[width=0.33\linewidth]{images/missing/medical_ib_disc6}
	}%
	\subfigure[\sc CAL500]{\hspace{-1mm}
		\includegraphics[width=0.33\linewidth]{images/missing/cal500_ib_disc6}
	}%
	\vspace{-2mm}\caption{\textbf{Missing labels - Imprecise Branching} Evolution of the average (\%) set-accuracy (top) and completeness (down) for each level of imprecision (a curve for each one) and a discretization $z=6$, with respect to the percentage of missing labels.}
\end{figure}








